Implementing Strassen's Algorithm with BLIS

We dispel with "street wisdom" regarding the practical implementation of Strassen's algorithm for matrix-matrix multiplication (DGEMM). Conventional wisdom: it is only practical for very large matrices. Our implementation is practical for small matrices. Conventional wisdom: the matrices being multiplied should be relatively square. Our implementation is practical for rank-k updates, where k is relatively small (a shape of importance for libraries like LAPACK). Conventional wisdom: it inherently requires substantial workspace. Our implementation requires no workspace beyond buffers already incorporated into conventional high-performance DGEMM implementations. Conventional wisdom: a Strassen DGEMM interface must pass in workspace. Our implementation requires no such workspace and can be plug-compatible with the standard DGEMM interface. Conventional wisdom: it is hard to demonstrate speedup on multi-core architectures. Our implementation demonstrates speedup over conventional DGEMM even on an Intel(R) Xeon Phi(TM) coprocessor utilizing 240 threads. We show how a distributed memory matrix-matrix multiplication also benefits from these advances.

==> 2-level.tex <==
\[
\begin{array}{ll}
%%
M_{0} = ( A_{0, 0} + A_{2, 2} + A_{1, 1} + A_{3, 3}  ) * ( B_{0, 0} +
B_{2, 2} + B_{1, 1} + B_{3, 3}  ); \\
~~~~~~~~~~~~C_{0, 0} += M_{0};
C_{1, 1} += M_{0};
C_{2, 2} += M_{0};
C_{3, 3} += M_{0};
\\
%%
M_{1} = ( A_{1, 0} + A_{3, 2} + A_{1, 1} + A_{3, 3}  ) * ( B_{0, 0} +
B_{2, 2}  );
~~~~~~~~~~~~
C_{1, 0} += M_{1};
C_{1, 1} -= M_{1};
C_{3, 2} += M_{1};
C_{3, 3} -= M_{1}; 
\\
%%
M_{2} = ( A_{0, 0} + A_{2, 2}  ) * ( B_{0, 1} + B_{2, 3} + B_{1, 1} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 1} += M_{2};
C_{1, 1} += M_{2};
C_{2, 3} += M_{2};
C_{3, 3} += M_{2};
\\
%%
M_{3} = ( A_{1, 1} + A_{3, 3}  ) * ( B_{1, 0} + B_{3, 2} + B_{0, 0} +
B_{2, 2}  );
~~~~~~~~~~~~
C_{0, 0} += M_{3};
C_{1, 0} += M_{3};
C_{2, 2} += M_{3};
C_{3, 2} += M_{3};
\\
%%
M_{4} = ( A_{0, 0} + A_{2, 2} + A_{0, 1} + A_{2, 3}  ) * ( B_{1, 1} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{4};
C_{0, 1} += M_{4};
C_{2, 2} -= M_{4};
C_{2, 3} += M_{4};
\\
%%
M_{5} = ( A_{1, 0} + A_{3, 2} + A_{0, 0} + A_{2, 2}  ) * ( B_{0, 0} +
B_{2, 2} + B_{0, 1} + B_{2, 3}  );
~~~~~~~~~~~~
C_{1, 1} += M_{5};
C_{3, 3} += M_{5};
\\
%%
M_{6} = ( A_{0, 1} + A_{2, 3} + A_{1, 1} + A_{3, 3}  ) * ( B_{1, 0} +
B_{3, 2} + B_{1, 1} + B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} += M_{6};
C_{2, 2} += M_{6};
\\
%%
M_{7} = ( A_{2, 0} + A_{2, 2} + A_{3, 1} + A_{3, 3}  ) * ( B_{0, 0} +
B_{1, 1}  );
~~~~~~~~~~~~
C_{2, 0} += M_{7};
C_{3, 1} += M_{7};
C_{2, 2} -= M_{7};
C_{3, 3} -= M_{7};
\\
%%
M_{8} = ( A_{3, 0} + A_{3, 2} + A_{3, 1} + A_{3, 3}  ) * ( B_{0, 0}
);
~~~~~~~~~~~~
C_{3, 0} += M_{8};
C_{3, 1} -= M_{8};
C_{3, 2} -= M_{8};
C_{3, 3} += M_{8};
\\
%%
M_{9} = ( A_{2, 0} + A_{2, 2}  ) * ( B_{0, 1} + B_{1, 1}  );
~~~~~~~~~~~~
C_{2, 1} += M_{9};
C_{3, 1} += M_{9};
C_{2, 3} -= M_{9};
C_{3, 3} -= M_{9};
\\
%%
M_{10} = ( A_{3, 1} + A_{3, 3}  ) * ( B_{1, 0} + B_{0, 0}  );
~~~~~~~~~~~~
C_{2, 0} += M_{10};
C_{3, 0} += M_{10};
C_{2, 2} -= M_{10};
C_{3, 2} -= M_{10};
\\
%%
M_{11} -= ( A_{2, 0} + A_{2, 2} + A_{2, 1} + A_{2, 3}  ) * ( B_{1, 1}
);
~~~~~~~~~~~~
C_{2, 0} -= M_{11};
C_{2, 1} += M_{11};
C_{2, 2} += M_{11};
C_{2, 3} -= M_{11};
\\
%%
M_{12} = ( A_{3, 0} + A_{3, 2} + A_{2, 0} + A_{2, 2}  ) * ( B_{0, 0} +
B_{0, 1}  );
~~~~~~~~~~~~
C_{3, 1} += M_{12};
C_{3, 3} -= M_{12};
\\
%%
M_{13} = ( A_{2, 1} + A_{2, 3} + A_{3, 1} + A_{3, 3}  ) * ( B_{1, 0} +
B_{1, 1}  );
~~~~~~~~~~~~
C_{2, 0} += M_{13};
C_{2, 2} -= M_{13};
\\
%%
M_{14} = ( A_{0, 0} + A_{1, 1}  ) * ( B_{0, 2} + B_{2, 2} + B_{1, 3} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 2} += M_{14};
C_{1, 3} += M_{14};
C_{2, 2} += M_{14};
C_{3, 3} += M_{14};
\\
%%
M_{15} = ( A_{1, 0} + A_{1, 1}  ) * ( B_{0, 2} + B_{2, 2}  );
~~~~~~~~~~~~
C_{1, 2} += M_{15};
C_{1, 3} -= M_{15};
C_{3, 2} += M_{15};
C_{3, 3} -= M_{15};
\\
%%
M_{16} = ( A_{0, 0}  ) * ( B_{0, 3} + B_{2, 3} + B_{1, 3} + B_{3, 3}
);
~~~~~~~~~~~~
C_{0, 3} += M_{16};
C_{1, 3} += M_{16};
C_{2, 3} += M_{16};
C_{3, 3} += M_{16};
\\
%%
M_{17} = ( A_{1, 1}  ) * ( B_{1, 2} + B_{3, 2} + B_{0, 2} + B_{2, 2}
);
~~~~~~~~~~~~
C_{0, 2} += M_{17};
C_{1, 2} += M_{17};
C_{2, 2} += M_{17};
C_{3, 2} += M_{17};
\\
%%
M_{18} -= ( A_{0, 0} + A_{0, 1}  ) * ( B_{1, 3} + B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 2} -= M_{18};
C_{0, 3} += M_{18};
C_{2, 2} -= M_{18};
C_{2, 3} += M_{18};
\\
%%
M_{19} = ( A_{1, 0} + A_{0, 0}  ) * ( B_{0, 2} + B_{2, 2} + B_{0, 3} +
B_{2, 3}  );
~~~~~~~~~~~~
C_{1, 3} += M_{19};
C_{3, 3} += M_{19};
\\
%%
M_{20} = ( A_{0, 1} + A_{1, 1}  ) * ( B_{1, 2} + B_{3, 2} + B_{1, 3} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 2} += M_{20};
C_{2, 2} += M_{20};
\\
%%
M_{21} = ( A_{2, 2} + A_{3, 3}  ) * ( B_{2, 0} + B_{0, 0} + B_{3, 1} +
B_{1, 1}  );
~~~~~~~~~~~~
C_{0, 0} += M_{21};
C_{1, 1} += M_{21};
C_{2, 0} += M_{21};
C_{3, 1} += M_{21};
\\
%%
M_{22} = ( A_{3, 2} + A_{3, 3}  ) * ( B_{2, 0} + B_{0, 0}  );
~~~~~~~~~~~~
C_{1, 0} += M_{22};
C_{1, 1} -= M_{22};
C_{3, 0} += M_{22};
C_{3, 1} -= M_{22};
\\
%%
M_{23} = ( A_{2, 2}  ) * ( B_{2, 1} + B_{0, 1} + B_{3, 1} + B_{1, 1}
);
~~~~~~~~~~~~
C_{0, 1} += M_{23};
C_{1, 1} += M_{23};
C_{2, 1} += M_{23};
C_{3, 1} += M_{23};
\\
%%
M_{24} = ( A_{3, 3}  ) * ( B_{3, 0} + B_{1, 0} + B_{2, 0} + B_{0, 0}
);
~~~~~~~~~~~~
C_{0, 0} += M_{24};
C_{1, 0} += M_{24};
C_{2, 0} += M_{24};
C_{3, 0} += M_{24};
\\
%%
M_{25} -= ( A_{2, 2} + A_{2, 3}  ) * ( B_{3, 1} + B_{1, 1}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{25};
C_{0, 1} += M_{25};
C_{2, 0} -= M_{25};
C_{2, 1} += M_{25};
\\
%%
M_{26} = ( A_{3, 2} + A_{2, 2}  ) * ( B_{2, 0} + B_{0, 0} + B_{2, 1} +
B_{0, 1}  );
~~~~~~~~~~~~
C_{1, 1} += M_{26};
C_{3, 1} += M_{26};
\\
%%
M_{27} = ( A_{2, 3} + A_{3, 3}  ) * ( B_{3, 0} + B_{1, 0} + B_{3, 1} +
B_{1, 1}  );
~~~~~~~~~~~~
C_{0, 0} += M_{27};
C_{2, 0} += M_{27};
\\
%%
M_{28} -= ( A_{0, 0} + A_{0, 2} + A_{1, 1} + A_{1, 3}  ) * ( B_{2, 2} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{28};
C_{1, 1} -= M_{28};
C_{0, 2} += M_{28};
C_{1, 3} += M_{28};
\\
%%
M_{29} -= ( A_{1, 0} + A_{1, 2} + A_{1, 1} + A_{1, 3}  ) * ( B_{2, 2}
);
~~~~~~~~~~~~
C_{1, 0} -= M_{29};
C_{1, 1} += M_{29};
C_{1, 2} += M_{29};
C_{1, 3} -= M_{29};
\\
%%
M_{30} -= ( A_{0, 0} + A_{0, 2}  ) * ( B_{2, 3} + B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 1} -= M_{30};
C_{1, 1} -= M_{30};
C_{0, 3} += M_{30};
C_{1, 3} += M_{30};
\\
%%
M_{31} -= ( A_{1, 1} + A_{1, 3}  ) * ( B_{3, 2} + B_{2, 2}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{31};
C_{1, 0} -= M_{31};
C_{0, 2} += M_{31};
C_{1, 2} += M_{31};
\\
%%
M_{32} = ( A_{0, 0} + A_{0, 2} + A_{0, 1} + A_{0, 3}  ) * ( B_{3, 3}
);
~~~~~~~~~~~~
C_{0, 0} += M_{32};
C_{0, 1} -= M_{32};
C_{0, 2} -= M_{32};
C_{0, 3} += M_{32};
\\
%%
M_{33} -= ( A_{1, 0} + A_{1, 2} + A_{0, 0} + A_{0, 2}  ) * ( B_{2, 2} +
B_{2, 3}  );
~~~~~~~~~~~~
C_{1, 1} -= M_{33};
C_{1, 3} += M_{33};
\\
%%
M_{34} -= ( A_{0, 1} + A_{0, 3} + A_{1, 1} + A_{1, 3}  ) * ( B_{3, 2} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{34};
C_{0, 2} += M_{34};
\\
%%
M_{35} = ( A_{2, 0} + A_{0, 0} + A_{3, 1} + A_{1, 1}  ) * ( B_{0, 0} +
B_{0, 2} + B_{1, 1} + B_{1, 3}  );
~~~~~~~~~~~~
C_{2, 2} += M_{35};
C_{3, 3} += M_{35};
\\
%%
M_{36} = ( A_{3, 0} + A_{1, 0} + A_{3, 1} + A_{1, 1}  ) * ( B_{0, 0} +
B_{0, 2}  );
~~~~~~~~~~~~
C_{3, 2} += M_{36};
C_{3, 3} -= M_{36};
\\
%%
M_{37} = ( A_{2, 0} + A_{0, 0}  ) * ( B_{0, 1} + B_{0, 3} + B_{1, 1} +
B_{1, 3}  );
~~~~~~~~~~~~
C_{2, 3} += M_{37};
C_{3, 3} += M_{37};
\\
%%
M_{38} = ( A_{3, 1} + A_{1, 1}  ) * ( B_{1, 0} + B_{1, 2} + B_{0, 0} +
B_{0, 2}  );
~~~~~~~~~~~~
C_{2, 2} += M_{38};
C_{3, 2} += M_{38};
\\
%%
M_{39} -= ( A_{2, 0} + A_{0, 0} + A_{2, 1} + A_{0, 1}  ) * ( B_{1, 1} +
B_{1, 3}  );
~~~~~~~~~~~~
C_{2, 2} -= M_{39};
C_{2, 3} += M_{39};
\\
%%
M_{40} = ( A_{3, 0} + A_{1, 0} + A_{2, 0} + A_{0, 0}  ) * ( B_{0, 0} +
B_{0, 2} + B_{0, 1} + B_{0, 3}  );
~~~~~~~~~~~~
C_{3, 3} += M_{40};
\\
%%
M_{41} = ( A_{2, 1} + A_{0, 1} + A_{3, 1} + A_{1, 1}  ) * ( B_{1, 0} +
B_{1, 2} + B_{1, 1} + B_{1, 3}  );
~~~~~~~~~~~~
C_{2, 2} += M_{41};
\\
%%
M_{42} = ( A_{0, 2} + A_{2, 2} + A_{1, 3} + A_{3, 3}  ) * ( B_{2, 0} +
B_{2, 2} + B_{3, 1} + B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} += M_{42};
C_{1, 1} += M_{42};
\\
%%
M_{43} = ( A_{1, 2} + A_{3, 2} + A_{1, 3} + A_{3, 3}  ) * ( B_{2, 0} +
B_{2, 2}  );
~~~~~~~~~~~~
C_{1, 0} += M_{43};
C_{1, 1} -= M_{43};
\\
%%
M_{44} = ( A_{0, 2} + A_{2, 2}  ) * ( B_{2, 1} + B_{2, 3} + B_{3, 1} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 1} += M_{44};
C_{1, 1} += M_{44};
\\
%%
M_{45} = ( A_{1, 3} + A_{3, 3}  ) * ( B_{3, 0} + B_{3, 2} + B_{2, 0} +
B_{2, 2}  );
~~~~~~~~~~~~
C_{0, 0} += M_{45};
C_{1, 0} += M_{45};
\\
%%
M_{46} -= ( A_{0, 2} + A_{2, 2} + A_{0, 3} + A_{2, 3}  ) * ( B_{3, 1} +
B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} -= M_{46};
C_{0, 1} += M_{46};
\\
%%
M_{47} = ( A_{1, 2} + A_{3, 2} + A_{0, 2} + A_{2, 2}  ) * ( B_{2, 0} +
B_{2, 2} + B_{2, 1} + B_{2, 3}  );
~~~~~~~~~~~~
C_{1, 1} += M_{47};
\\
%%
M_{48} = ( A_{0, 3} + A_{2, 3} + A_{1, 3} + A_{3, 3}  ) * ( B_{3, 0} +
B_{3, 2} + B_{3, 1} + B_{3, 3}  );
~~~~~~~~~~~~
C_{0, 0} += M_{48};
\end{array}
\]


==> fig_VpW.tex <==
%%\begin{figure*}[tb!]
\begin{figure}[p]

\begin{center}
%\includegraphics[width=0.75\textwidth]{Pack3.pdf}
\includegraphics[width=0.65\textwidth]{Pictures/LayersVpW.pdf}
\end{center}

\caption{
Modification to Figure~\ref{fig:gemm} that shows how the basic 
implementation of $ C = A B + C $ can be modified to compute $ C = ( V
+ W ) B $ instead.
}
\label{fig:VpW}
\end{figure}



==> fig_XpY.tex <==
%%\begin{figure*}[tb!]
\begin{figure}[p]

\begin{center}
%\includegraphics[width=0.75\textwidth]{Pack3.pdf}
\includegraphics[width=0.65\textwidth]{Pictures/LayersXpY.pdf}
\end{center}

\caption{
Modification to Figure~\ref{fig:gemm} that shows how the basic 
implementation of $ C = A B + C $ can be modified to compute $ C = A(
X + Y ) $ instead.
}
\label{fig:XpY}
\end{figure}



==> fig_XpY_VpW.tex <==
%%\begin{figure*}[tb!]
\begin{figure}[p]

\begin{center}
\includegraphics[width=0.65\textwidth]{Pictures/LayersXpYVpW.pdf}
\end{center}

\caption{
Modification to Figure~\ref{fig:gemm} that shows how the basic 
implementation of $ C = A B + C $ can be modified to compute $ C = (X+Y)(
V+W ) $ instead. 
}
\label{fig:XpY_VpW}
\end{figure}



==> fig_gemm.tex <==
%%\begin{figure*}[tb!]
\begin{figure}[tb!]

\begin{center}
%\includegraphics[width=0.75\textwidth]{Pack3.pdf}
\includegraphics[width=0.65\textwidth]{Pictures/LayeringOriginal.pdf}
\end{center}

\caption{
Illustration from~\cite{FLAWN66} of the various levels of blocking and related
packing when implementing {\sc gemm} in the style
of~\cite{Goto:2008:AHP}.
The bottom layer shows the general {\sc gemm} and exposes the special
case where $ k = k_c $ (known as a rank-k update, with $ k = k_c $).
The top layer shows the micro-kernel upon which the BLIS implementation
is layered.
Here, $ m_c $ and $ k_c $ serve as cache block sizes used by the
higher-level blocked algorithms to partition the matrix problem down to
a so-called ``block-panel'' subproblem (depicted in the middle of the
diagram), implemented in BLIS as a portable macro-kernel.
(The middle layer corresponds to the ``inner kernel'' in the GotoBLAS.)  
Similarly, $ m_r $ and $ n_r $ serve as register block sizes for the
micro-kernel in the $ m $ and $ n $ dimensions, respectively, which also
correspond to the length and width of the individual packed panels of
matrices $ \tilde A_i $ and $ \tilde B $, respectively.
}
\label{fig:gemm}
\end{figure}



==> loops.tex <==
\newcommand{\plusequal}{ \!\!\begin{array}{c}
     \tiny +\\[-0.06in] \tiny =\end{array} \!\!}
\newcommand{\plusequalo}{ \!\!\begin{array}{c}
     \tiny +\\[-0.09in] \tiny =\end{array} \!\!}

\begin{figure*}[t!]
\begin{tabular}{@{}l@{}}
\begin{minipage}{\textwidth}
$
\begin{array}{l}
\mbox{\bf for } j_c = 0, \dots , n-1 \mbox{\bf ~in steps of } n_c \\
~~ \mbox{\bf for } p_c = 0, \ldots, k-1 \mbox{\bf ~in steps of } k_c \\
~~~~ \mbox{\bf for } i_c = 0, \ldots, m-1 \mbox{\bf ~in steps of } m_c \\
~~~~~~ \mbox{\bf for } j_r = 0, \ldots, n_c-1 \mbox{\bf ~in steps of } n_r \\
~~~~~~~~  \left.
\begin{array}{@{} l @{\hspace{-0.05in}}}
\color{red} \mbox{\bf  for } i_r = 0, \ldots, m_c-1 \mbox{\bf ~in steps of } m_r \\
~~  \left.
 \begin{array}{@{} l @{\hspace{-0.05in}}}
   C( i_r  \!\! : \! i_r \! + \! m_r\!-\!1, j_r \!\! : \! j_r \! + \! n_r\!-\!1 ) \plusequalo  \cdots
%%%\\
%%%~~  A( i_r \! : \! i_r \! : \! m_r\!-\!1, p_c \! : \! p_c+k_c-1 ) \times  \\
%%%~~~~ B( p_c \! : \! p_c+k_c-1, j_r \! : \! j_r+n_r\!-\!1 ) 
\end{array}  \right\}
\begin{array}{@{}c}
\includegraphics[width=0.95in]{Pictures/microkernel.pdf} 
\end{array}
\\
\mbox{\bf \color{red} endfor} \\
\end{array} 
\color{red}  \right\} 
\begin{array}{c}
\includegraphics[width=1.3in]{Pictures/i1loop.pdf} \\
\mbox{(loop around micro-kernel)}
\end{array}
\\
~~~~~~ \mbox{\bf endfor} \\
~~~~ \mbox{\bf endfor} \\
~~ \mbox{\bf endfor} \\
\mbox{\bf endfor} 
\end{array}
$
\end{minipage}
\\
\\
\begin{minipage}{0.95\textwidth}
$
\begin{array}{l}
\mbox{\bf for } j_c = 0, \dots , n-1 \mbox{\bf ~in steps of } n_c \\
~~ \mbox{\bf for } p_c = 0, \ldots, k-1 \mbox{\bf ~in steps of } k_c \\
~~~~ \mbox{\bf for } i_c = 0, \ldots, m-1 \mbox{\bf ~in steps of } m_c
\\[0.1in]
~~~~~~  \left.
 \begin{array}{@{} l @{\hspace{-0.05in}}}
\color{red} \mbox{\bf  for } j_r = 0, \ldots, n_c-1 \mbox{\bf ~in steps of } n_r \\
\footnotesize
~~\mbox{\bf for } i_r = 0, \ldots, m_c-1 \mbox{\bf ~in steps of } m_r \\
\footnotesize
~~~~   C( i_r \!\! : \! i_r \! + \! m_r\!-\!1, j_r \!\! : \! j_r \! + \! n_r\!-\!1 ) \plusequal  \cdots
%%%\\
%%%~~~~~~  A( i_r \! : \! i_r \! : \! m_r\!-\!1, p_c \! : \! p_c+k_c-1 ) \times  \\
%%%~~~~~~~~ B( p_c \! : \! p_c+k_c-1, j_r \! : \! j_r+n_r\!-\!1 )  
\\
\footnotesize
~~\mbox{\bf endfor} \\
\mbox{\bf \color{red} endfor} 
\end{array}
\color{red}  \right\}
\begin{array}{@{}c@{}}
\includegraphics[width=3in]{Pictures/j1loop.pdf}
\end{array}
\\
\\[-0.05in]
~~~~ \mbox{\bf endfor} \\
~~ \mbox{\bf endfor} \\
\mbox{\bf endfor} 
\end{array}
$
\end{minipage}
\\
\\
\begin{minipage}{0.95\textwidth}
$
\begin{array}{l}
\mbox{\bf for } j_c = 0, \dots , n-1 \mbox{\bf ~in steps of } n_c \\
~~ \mbox{\bf for } p_c = 0, \ldots, k-1 \mbox{\bf ~in steps of } k_c
\\[0.1in]
~~~~ 
\left.
 \begin{array}{@{} l @{\hspace{-0.05in}}}
\color{red}
\mbox{\bf for } i_c = 0, \ldots, m-1 \mbox{\bf ~in steps of } m_c
\\
\footnotesize
~~\mbox{\bf for } j_r = 0, \ldots, n_c-1 \mbox{\bf ~in steps of } n_r \\
\footnotesize
~~~~\mbox{\bf for } i_r = 0, \ldots, m_c-1 \mbox{\bf ~in steps of } m_r \\
\footnotesize
~~~~~~   C( i_r \!\! : \! i_r \! + \! m_r\!-\!1, j_r \!\! : \! j_r \! + \!
n_r\!-\!1 ) \plusequal  \cdots
%%%\\
%%%~~~~~~~~  A( i_r \! : \! i_r \! : \! m_r\!-\!1, p_c \! : \! p_c+k_c-1 ) \times  \\
%%%~~~~~~~~~~ B( p_c \! : \! p_c+k_c-1, j_r \! : \! j_r+n_r\!-\!1 )  
\\
\footnotesize
~~~~\mbox{\bf endfor} \\
\footnotesize
~~\mbox{\bf endfor} 
\\
\mbox{\bf \color{red} endfor} \\
\end{array}
\color{red}  \right\}
\begin{array}{c}
\includegraphics[width=3in]{Pictures/i0loop.pdf}
\end{array}
\\[-0.05in]
\\
~~ \mbox{\bf endfor} \\
\mbox{\bf endfor} 
\end{array}
$
\end{minipage}
\end{tabular}
\caption{Illustration of the three inner-most loops. The loops idexed
  by $ i_r $ and $ j_r $ are the loops that were hidden inside 
  the GotoBLAS inner kernel.}
\label{fig:inner_three_loops}
\end{figure*}

%$
%\end{minipage}
%\\
%\\
%\begin{minipage}{0.95\textwidth}
%$
%\begin{array}{l}
%\mbox{\bf for } j_c = 0, \dots , n-1 \mbox{\bf ~in steps of } n_c \\[0.1in]
%~~ 
%\left.
% \begin{array}{@{} l @{\hspace{-0.05in}}}
%\color{red} \mbox{\bf  for } p_c = 0, \ldots, k-1 \mbox{\bf ~in steps of } k_c
%\\
%\footnotesize
%~~\mbox{\bf for } i_c = 0, \ldots, m-1 \mbox{\bf ~in steps of } m_c
%\\
%\footnotesize
%~~~~\mbox{\bf for } j_r = 0, \ldots, n_c-1 \mbox{\bf ~in steps of } n_r \\
%\footnotesize
%~~~~~~\mbox{\bf for } i_r = 0, \ldots, m_c-1 \mbox{\bf ~in steps of } m_r \\
%\footnotesize
%~~~~~~~~   C( i_r \!\! : \! i_r \! + \! m_r\!-\!1, j_r \!\! : \! j_r \! +
%\! n_r\!-\!1 ) \plusequal  \cdots
%%%%\\
%%%%~~~~~~~~  A( i_r \! : \! i_r \! : \! m_r\!-\!1, p_c \! : \! p_c+k_c-1 ) \times  \\
%%%%~~~~~~~~~~ B( p_c \! : \! p_c+k_c-1, j_r \! : \! j_r+n_r\!-\!1 )  
%\\
%\footnotesize
%~~~~~~\mbox{\bf endfor} \\
%\footnotesize
%~~~~\mbox{\bf endfor} 
%\\
%\footnotesize
%~~\mbox{\bf endfor} \\
%\mbox{\bf \color{red} endfor} \\
%\end{array}
%\color{red}  \right\}
% \begin{array}{@{} l @{\hspace{-0.05in}}}
%\includegraphics[width=3.25in]{Pictures/p0loop1.pdf}
%\end{array}
%\\[-0.05in]
%\\
%\mbox{\bf endfor} 
%\end{array}
%$
%\end{minipage}
%\\
%\\
%\begin{minipage}{0.95\textwidth}
%$
%\begin{array}{l}
%\left.
% \begin{array}{@{} l @{\hspace{-0.05in}}}
%\color{red} \mbox{\bf for } j_c = 0, \dots , n-1 \mbox{\bf ~in steps of } n_c \\[0.1in]
%\footnotesize
%~~
%\mbox{\bf for } p_c = 0, \ldots, k-1 \mbox{\bf ~in steps of } k_c
%\\
%\footnotesize
%~~~~\mbox{\bf for } i_c = 0, \ldots, m-1 \mbox{\bf ~in steps of } m_c
%\\
%\footnotesize
%~~~~~~\mbox{\bf for } j_r = 0, \ldots, n_c-1 \mbox{\bf ~in steps of } n_r \\
%\footnotesize
%~~~~~~~~\mbox{\bf for } i_r = 0, \ldots, m_c-1 \mbox{\bf ~in steps of } m_r \\
%\footnotesize
%~~~~~~~~~~   C( i_r \!\! : \! i_r \! + \! m_r\!-\!1, j_r \!\! : \! j_r \!
%+ \! n_r\!-\!1 ) \plusequal  \cdots
%%%%\\
%%%%~~~~~~~~  A( i_r \! : \! i_r \! : \! m_r\!-\!1, p_c \! : \! p_c+k_c-1 ) \times  \\
%%%%~~~~~~~~~~ B( p_c \! : \! p_c+k_c-1, j_r \! : \! j_r+n_r\!-\!1 )  
%\\
%\footnotesize
%~~~~~~~~\mbox{\bf endfor} \\
%\footnotesize
%~~~~~~\mbox{\bf endfor} 
%\\
%\footnotesize
%~~~~\mbox{\bf endfor} \\
%\footnotesize
%~~\mbox{\bf endfor} \\
%\mbox{\bf \color{red} endfor} 
%\end{array}
%\color{red}  \right\}
% \begin{array}{@{} l @{\hspace{-0.05in}}}
%\includegraphics[width=3.5in]{Pictures/j0loop.pdf}
%\end{array}
%\\[-0.05in]
%\end{array}
%$
%\end{minipage}
%\end{tabular}
%\caption{Illustration of the three outer-most loops (around what was
%  Goto's inner kernel).}
%\label{fig:outer_three_loops}
%\end{figure*}
%
%


==> myperformance.tex <==
\input setup


==> new_table.tex <==
\begin{figure*}[tb!]
	\begin{tabular}{l I c @{=} c @{$+$} c c @{$+$}
			c @{$\cdot$} c @{$+$}
			c @{$\cdot$} c @{$+$}
			c @{$\cdot$} c @{$+$}
			c @{$\cdot$} c @{$+$}
			c @{$\cdot$} c @{$+$}
			c @{$\cdot$} c  } \hline
Variation &		$ T_m $ & 
$ T_a^\times $ &
$ N_m^{A_\times} $ & $ T_m^{A_\times} $ &  
		$ N_m^{A_+} $ & $ T_m^{A_+} $ &
		$ N_m^{B_\times} $ & $ T_m^{B_\times} $ &
		$ N_m^{B_+} $ & $ T_m^{B_+} $ &
		$ N_m^{C_\times} $ & $ T_m^{C_\times} $ &
		$ N_m^{C_+} $ & $ T_m^{C_+} $ \\ \whline
		{\tt dgemm} & & $ 2 m n k $ \\ \hline
		1-level Strassen &
		& $7 \times 2 \frac{m}{2} \frac{n}{2} \frac{k}{2} $ &
		$ 7 $ & $ \frac{m}{2}\frac{k}{2}\lceil\frac{n}{2n_c}\rceil$
		
	\end{tabular}
\end{figure*}

==> setup_old.tex <==
\begin{figure*}[htp!]
	\centering
	%%  \includegraphics[width=0.32\textwidth]{figures/outsquare_1core.pdf}
	%%  \includegraphics[width=0.32\textwidth]{figures/outrankk_1core.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outfixk_1core.pdf}
	%%  \includegraphics[width=0.32\textwidth]{figures/outfixk1024_1core.pdf}
	%% \\
	\includegraphics[width=0.43\textwidth]{figures/outsquare_5core.pdf}
	\includegraphics[width=0.43\textwidth]{figures/outsquare_10core.pdf}
	\includegraphics[width=0.43\textwidth]{figures/outrankk_5core.pdf}
	\includegraphics[width=0.43\textwidth]{figures/outrankk_10core.pdf}
	%\includegraphics[width=0.43\textwidth]{figures/outfixk_5core.pdf}
	\includegraphics[width=0.43\textwidth]{figures/outfixk1024_5core.pdf}
	\includegraphics[width=0.43\textwidth]{figures/outfixk1024_10core.pdf}
	\caption{Performance of the various implementations on an Intel Xeon E5 2680 v2 (Ivybridge) processor.  
		%The first row 
		%The X-axis is the dimension size from 4 to 1028, and
		%the Y-axis is GFLOPS where the theoretical peak performance for 1 core, 5 core, 10 core are
		%248 GFLOPS ($8 \times 3.1 \times 10$).
	}
	\label{fig:single_node}
\end{figure*} 

We give details on the performance experiments for our implementations.
The current version of \strassen\ \dgemm\ was designed for the Intel Sandy-Bridge/Ivy-Bridge processor and Intel 
Intel Xeon Phi Coprocessor (MIC Architecture, Knights Corner).  In addition, we incorporated the \ABCstrassen\ in a distributed memory \gemm.

\subsection{Single node experiments}
\label{sec:perf:single_node}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Moved to implementation.tex
\subsubsection*{Implementation}
%
%For our implementations, components from the \BLIS{} framework were modified.  We refer to the submatrices in \figref{fig:side-by-side} as we describe these.
%
%\begin{itemize}
%	\item The reference \BLIS{} routines that pack $ \widetilde B_p $ and $ \widetilde A_i $ were modified to incorporate the addition (with appropriate scaling) of two to four matrices.  
%	The reference \BLIS{} pack routines parallelize these operations when multiple threads are used as described in~\cite{}.  Our modified routines inherit this parallelization.
%	\item
%	The optimized microkernels for each of the target architectures were modified so that the resulting $ m_r \times n_r $ microblock of $ C $ is added to up to four submatrices of $ C $.
%	\item
%	The loops in \BLIS{} that implement \gemm\ were modified to track through multiple matrices (up to four).
%\end{itemize}
%Together, this allowed us to implement the Integrated Strassen algorithm described earlier in this paper.
%
%For comparison, a number of additional implementations were created:
%\begin{itemize}
%	\item 
%	Naive Strassen implementations were implementated that implement Strassen's algorithm in a straight forward way, with intermediate temporary matrices and calls to the traditional BLAS \dgemm\ routine.
%	\item
%	A two level hybrid implementation that performs one level of a naive Strassen implementation and then uses one level of the Integrated Strassen implementation for the second level.
%\end{itemize}
%In addition to testing the performance of the various implementations of one-level and two-level \strassen, we also tested a two-level Hybrid \strassen, which performs one level of a naive \strassen\ implementation and then uses a one-level \ABCstrassen\ implementation for the second level.
%These allow us to assess the trade-offs between the various members of the family of algorithms.

The implementations are in {\tt C}, utilizing {\tt SSE2} and {\tt AVX} intrinsics and assembly, compiled with the Intel {\tt C} compiler version 15.0.3 with optimization flag {\tt -O3}. 
In addition, we compare against the standard \BLIS\  implementation (Version 0.1.8) from which our implementations were derived as well as MKL's \dgemm\ (MKL Release Version 11.2.3).


\subsubsection*{Target architecture}

We measure the CPU performance results on the Maverick system at the Texas Advanced Computing Center (TACC).  Each node of that system consists of a  
dual-socket Intel Xeon E5-2680 v2 (Ivy Bridge) processors with 12.8GB/core of memory
(Peak Bandwidth: 59.7 GB/s) and a three-level cache: 32KB L1 data cache, 256KB L2 cache and 25.6MB L3 cache.
The stable CPU clockrate is 3.54GHz for when a single core is utilized (28.32 GFLOPS peak, marked in the graphs) and 3.10GHz when five or more cores are in use (24.8 GLOPS/core peak). 
To make sure the computation and the memory allocation all reside on 
the same socket, we use {\tt KMP\_AFFINITY=compact}.

We chose the parameters $n_R=4$, $m_R=8$, $k_C=256$, $n_C=4096$ and $m_C=96$. This makes the size of the packing buffer
$ \widetilde A_i $ 192KB and 
$ \widetilde B_p $ 8192KB, which then fit the L2 cache and L3 cache, respectively.  These parameters are consistent with parameters used for the standard \BLIS\ \dgemm\ implementation for this architecture.

Each socket consists of 10 cores, allowing us to also perform multi-threaded experiments.  Parallelization 
was implemented mirroring that described in~\cite{BLIS3}, using OpenMP directives that parallelized the third loop around the microkernel in Figure~\ref{fig:side_by_side}.  

\subsubsection*{Results}




\NoShow{
	\begin{figure*}[htp]
	\centering
	\includegraphics[width=0.32\textwidth]{figures/outsquare_1core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outrankk_1core.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outfixk_1core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outfixk1024_1core.pdf}
	\\
	\includegraphics[width=0.32\textwidth]{figures/outsquare_5core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outrankk_5core.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outfixk_5core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outfixk1024_5core.pdf}
	\\
	\includegraphics[width=0.32\textwidth]{figures/outsquare_10core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outrankk_10core.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outfixk_10core.pdf}
	\includegraphics[width=0.32\textwidth]{figures/outfixk1024_10core.pdf}
	\caption{Performance of the various implementations on an Intel Xeon E5 2680 v2 (Ivybridge) processor.  Notice that the range of the y-axis does not start at zero to make the graphs more readable.  For single core experiments, 28.32 marks theoretical peak performance.
		%The first row 
		%The X-axis is the dimension size from 4 to 1028, and
		%the Y-axis is GFLOPS where the theoretical peak performance for 1 core, 5 core, 10 core are
		%248 GFLOPS ($8 \times 3.1 \times 10$).
	}
	\label{fig:single_node}
\end{figure*} 
}

Results  are presented in \figref{fig:single_node} (top row).
As expected, eventually two-level \ABXstrassen\ performs best, handily beating conventional \dgemm.  
The exception is the case where $ k $ is fixed to equal $ 1024 = 4 \times k_C $, which is the natural blocking size for a two-level \strassen\ based on our ideas.  For those experiments \ABCstrassen\ wins out, as expected.

%The distributed me
We also report in \figref{fig:single_node} results for five and ten cores, all within the same socket.   We do not report results for twenty cores, since this resulted in a substantial performance reduction for all our implementations, including the standard \BLIS\ \dgemm, relative to the MKL \dgemm.  This exposed a performance bug in \BLIS\ that has been reported.

When using many cores, memory bandwidth contention affects the performance of the various \strassen\ implementations, reducing the benefits relative to a standard \dgemm\ implementation.  


\subsection{Many-core experiments}
To examine whether the techniques scale to a large number of cores, we ported on implementation of one-level \ABCstrassen\ to the Intel Xeon Phi (KNC).

\subsubsection*{Implementation}

The implementations of \BLIS\ and \ABCstrassen\ are in {\tt C} and {\tt AVX512} intrinsics and assembly, compiled with the Intel {\tt C} compiler version 15.0.2 with optimization flag {\tt -mmic -O3}.  The \BLIS\ and \ABCstrassen\ both parallelize the second and third loop around the micro-kernel, as described for \BLIS\ in~\cite{BLIS3}.



\subsubsection*{Target architecture}

We ran the Xeon Phi (KNC) performance experiments on the Coprocessor SE10P incorporated into nodes of the Stampede system at TACC. This coprocessor
has a peak performance of 1056GFLOPS (60 cores/240 threads used by BLIS) and 8GB of GDDR5 DRAM with a peak bandwidth of 352GB/s. It has 512KB L2 cache, but no L3 cache.

We choose the parameters $n_R=8$, $m_R=30$, $k_C=240$, $n_C=14400$ and $m_C=120$. This makes the size of the packing buffer
$ \widetilde A_i $ 225KB and 
$ \widetilde B_p $ 27000KB, which fits L2 cache and main memory separately (no L3 cache on MIC).  These choices are consistent with those used by \BLIS\ for this architecture.

\subsubsection*{Results}

As illustrated in \figref{fig:mic}, relative to the \BLIS\ \dgemm\ implementation, the one-level \ABCstrassen\ shows a nontrivial improvement for a rank-k update with a fixed (large) matrix $ C $.  While the \BLIS\ implementation on which our implementation of \ABCstrassen\ used to be highly competitive with MKL's \dgemm\ (as reported in~\cite{BLIS3}), 
recent improvements in that library demonstrate that the \BLIS\ implementation needs an update.  We don't think there is a fundamental reason why our observations cannot be used to similarly accelerate MKL's \dgemm.

%This is also predicted by our performance model in { section }.


\begin{figure}[!tp]
	\centering
	%\includegraphics[width=0.32\textwidth]{figures/outsquare_mic.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outrankk_mic.pdf}
	%\includegraphics[width=0.32\textwidth]{figures/outfixk_mic.pdf}
	\includegraphics[width=0.43\textwidth]{figures/mic_rankk.pdf}
	\caption{Performance of the various implementations on an Intel Xeon Phi (KNC) processor (up to 61 cores with 244 threads).
		%The first row 
		%The X-axis is the dimension size from 4 to 1028, and
		%the Y-axis is GFLOPS where the theoretical peak performance for 1 core, 5 core, 10 core are
		%248 GFLOPS ($8 \times 3.1 \times 10$).
	}
	\label{fig:mic}
\end{figure} 



\subsection{Distributed memory experiments}

Finally, we demonstrate how the \ABCstrassen\ implementation can be used to accelerate a distributed memory implementation of \dgemm.
\subsubsection*{Implementation}

We implemented the Scalable Universal Matrix Multiplication Algorithm (SUMMA)~\cite{SUMMA} with MPI.  This algorithm distributes the algorithm to a mesh of MPI processes using a 2D blocked distribution.  The multiplication
is broken down into a sequence of rank-b updates,%
{\footnotesize%
\begin{eqnarray*}
C &:=& A B + C = \left(\begin{array}{c | c | c }
A_0 & \cdots & A_{K-1}
\end{array}
\right)
\left(
\begin{array}{c}
B_0 \\ \hline
\vdots \\ \hline
B_{K-1}
\end{array}
\right) + C \\
&=&
A_0 B_0 + \cdots + A_{K-1} B_{K-1} + C
\end{eqnarray*}%
}%
where each $ A_p $ consists of (approximately) $ b $ columns and each $ B_p $ consists of (approximately) $ b $ rows.
For each rank-b update  $ A_p $ is  broadcast within rows of the mesh and  $ B_p $ is broadcast within columns of the mesh, after which local a rank-b update with the arriving submatrices is performed to update a the local block of $ C $.  

\subsubsection*{Target architecture}

The distributed memory experiments were performed on the same machine described in Section~\ref{sec:perf:single_node}, using the 
{\tt mvapich2} version 2.1~\cite{MVAPICH2} implementation of MPI.
Each node has two socket, and each socket has ten cores.  

\begin{figure}[!tp]
	\centering
	\includegraphics[width=0.43\textwidth]{figures/mpi_square.pdf}
	\caption{Performance of the various implementations on distributed memory (weak scalability).
	}
	\label{fig:summa}
\end{figure} 

\subsubsection*{Results}
Figure~\figref{fig:summa} reports weak scalability.
For these experiments we chose the MPI mesh of processes to be square, with one MPI process per socket, and attained thread parallelism among the ten cores in a socket within BLIS, MKL, or one of our \strassen\ implementations.

It is well-known that the SUMMA algorithm is weakly scalable in the sense that efficiency essentially remains constant if the local memory dedicated to matrices $ A $, $ B $, $ C $, and temporary buffers is kept constant. 
For this reason, the local problem size is fixed to equal $m=k=n=16000$ so that the global problem becomes $ m=k=n=16000\times N $ when an $ N \times N $ mesh of sockets (MPI processes) is utilized. 
As expected, the graph shows that the SUMMA algorithm is weakly scalable regardless of which local \gemm\ algorithm is used.
The local computation within the SUMMA algorithm matches the shape for which \ABCstrassen\ is a natural choice when the rank-k updates are performed with $ b = 1024 $.  For this reason, the level-1 and level-2 \ABCstrassen\ implementations achieve the best performance.

What this experiment shows is that the benefit of using \strassen\ can be easily transfered to other algorithms that are rich in large rank-k updates.







==> twolevels_new.tex <==
\begin{figure}[t!]
~
\vspace{-0.05in}
{\footnotesize%
%{\tiny%
\[
\begin{array}{|l @{} l @{} l @{} l @{} l|} \hline
%
\multicolumn{5}{|l|}{
	M_{0} = ( A_{0, 0} \!+\! A_{2, 2} \!+\! A_{1, 1} \!+\! A_{3, 3}  )  ( B_{0, 0} +
B_{2, 2} \!+\! B_{1, 1} \!+\! B_{3, 3}  );
} \\
~~~~~ &
 C_{0, 0} +\!\!= M_{0};
&
C_{1, 1} +\!\!= M_{0};
&
C_{2, 2} +\!\!= M_{0};
& 
C_{3, 3} +\!\!= M_{0};
\\
\multicolumn{5}{|l|}{
	M_{1}  =  ( A_{1, 0} \!+\! A_{3, 2} \!+\! A_{1, 1} \!+\! A_{3, 3}  )  ( B_{0, 0} +
B_{2, 2}  );
}
\\
&
  
C_{1, 0} +\!\!= M_{1};
&
C_{1, 1} -\!\!= M_{1};
&
C_{3, 2} +\!\!= M_{1};
&
C_{3, 3} -\!\!= M_{1}; 
\\
%%
\multicolumn{5}{|l|}{
M_{2}  =  ( A_{0, 0} \!+\! A_{2, 2}  )  ( B_{0, 1} \!+\! B_{2, 3} \!+\! B_{1, 1} +
B_{3, 3}  );
} \\
&
C_{0, 1} +\!\!= M_{2};
&
C_{1, 1} +\!\!= M_{2};
&
C_{2, 3} +\!\!= M_{2};
&
C_{3, 3} +\!\!= M_{2};
\\
%%
\multicolumn{5}{|l|}{
M_{3}  =  ( A_{1, 1} \!+\! A_{3, 3}  )  ( B_{1, 0} \!+\! B_{3, 2} \!+\! B_{0, 0} +
B_{2, 2}  );
}\\
&
C_{0, 0} +\!\!= M_{3};
&
C_{1, 0} +\!\!= M_{3};
&
C_{2, 2} +\!\!= M_{3};
&
C_{3, 2} +\!\!= M_{3};
\\
%%
\multicolumn{5}{|l|}{
M_{4}  =  ( A_{0, 0} \!+\! A_{2, 2} \!+\! A_{0, 1} \!+\! A_{2, 3}  )  ( B_{1, 1} +
B_{3, 3}  );
} \\
&
C_{0, 0} -\!\!= M_{4};
&
C_{0, 1} +\!\!= M_{4};
&
C_{2, 2} -\!\!= M_{4};
&
C_{2, 3} +\!\!= M_{4};
\\
%%
\multicolumn{5}{|l|}{
M_{5}  =  ( A_{1, 0} \!+\! A_{3, 2} \!+\! A_{0, 0} \!+\! A_{2, 2}  )  ( B_{0, 0} +
B_{2, 2} \!+\! B_{0, 1} \!+\! B_{2, 3}  );
} \\
&
C_{1, 1} +\!\!= M_{5};
&
C_{3, 3} +\!\!= M_{5};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{6}  =  ( A_{0, 1} \!+\! A_{2, 3} \!+\! A_{1, 1} \!+\! A_{3, 3}  )  ( B_{1, 0} +
B_{3, 2} \!+\! B_{1, 1} \!+\! B_{3, 3}  );
} \\
&
C_{0, 0} +\!\!= M_{6};
&
C_{2, 2} +\!\!= M_{6};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{7}  =  ( A_{2, 0} \!+\! A_{2, 2} \!+\! A_{3, 1} \!+\! A_{3, 3}  )  ( B_{0, 0} +
B_{1, 1}  );
} \\
&
C_{2, 0} +\!\!= M_{7};
&
C_{3, 1} +\!\!= M_{7};
&
C_{2, 2} -\!\!= M_{7};
&
C_{3, 3} -\!\!= M_{7};
\\
\NoShow{
%%
\multicolumn{5}{|l|}{
M_{8}  =  ( A_{3, 0} \!+\! A_{3, 2} \!+\! A_{3, 1} \!+\! A_{3, 3}  )  ( B_{0, 0}
);
} \\
&
C_{3, 0} +\!\!= M_{8};
&
C_{3, 1} -\!\!= M_{8};
&
C_{3, 2} -\!\!= M_{8};
&
C_{3, 3} +\!\!= M_{8};
\\
%%
\multicolumn{5}{|l|}{
M_{9}  =  ( A_{2, 0} \!+\! A_{2, 2}  )  ( B_{0, 1} \!+\! B_{1, 1}  );
} \\
&
C_{2, 1} +\!\!= M_{9};
&
C_{3, 1} +\!\!= M_{9};
&
C_{2, 3} -\!\!= M_{9};
&
C_{3, 3} -\!\!= M_{9};
\\
%%
\multicolumn{5}{|l|}{
M_{10}  =  ( A_{3, 1} \!+\! A_{3, 3}  )  ( B_{1, 0} \!+\! B_{0, 0}  );
} \\
&
C_{2, 0} +\!\!= M_{10};
&
C_{3, 0} +\!\!= M_{10};
&
C_{2, 2} -\!\!= M_{10};
&
C_{3, 2} -\!\!= M_{10};
\\
%%
M_{11} = ( A_{2, 0} \!+\! A_{2, 2} \!+\! A_{2, 1} \!+\! A_{2, 3}  )  ( B_{1, 1}
); &
  
C_{2, 0} -\!\!= M_{11};
&
C_{2, 1} +\!\!= M_{11};
&
C_{2, 2} +\!\!= M_{11};
&
C_{2, 3} -\!\!= M_{11};
\\
%%
M_{12}  =  ( A_{3, 0} \!+\! A_{3, 2} \!+\! A_{2, 0} \!+\! A_{2, 2}  )  ( B_{0, 0} +
B_{0, 1}  );
&
  
C_{3, 1} +\!\!= M_{12};
&
C_{3, 3} -\!\!= M_{12};
&
&
\\
%%
M_{13}  =  ( A_{2, 1} \!+\! A_{2, 3} \!+\! A_{3, 1} \!+\! A_{3, 3}  )  ( B_{1, 0} +
B_{1, 1}  );
&
  
C_{2, 0} +\!\!= M_{13};
&
C_{2, 2} -\!\!= M_{13};
&
&
\\
%%
M_{14}  =  ( A_{0, 0} \!+\! A_{1, 1}  )  ( B_{0, 2} \!+\! B_{2, 2} \!+\! B_{1, 3} +
B_{3, 3}  );
&
  
C_{0, 2} +\!\!= M_{14};
&
C_{1, 3} +\!\!= M_{14};
&
C_{2, 2} +\!\!= M_{14};
&
C_{3, 3} +\!\!= M_{14};
\\
%%
M_{15}  =  ( A_{1, 0} \!+\! A_{1, 1}  )  ( B_{0, 2} \!+\! B_{2, 2}  );
&
  
C_{1, 2} +\!\!= M_{15};
&
C_{1, 3} -\!\!= M_{15};
&
C_{3, 2} +\!\!= M_{15};
&
C_{3, 3} -\!\!= M_{15};
\\
%%
M_{16}  =  ( A_{0, 0}  )  ( B_{0, 3} \!+\! B_{2, 3} \!+\! B_{1, 3} \!+\! B_{3, 3}
);
&
  
C_{0, 3} +\!\!= M_{16};
&
C_{1, 3} +\!\!= M_{16};
&
C_{2, 3} +\!\!= M_{16};
&
C_{3, 3} +\!\!= M_{16};
\\
%%
M_{17}  =  ( A_{1, 1}  )  ( B_{1, 2} \!+\! B_{3, 2} \!+\! B_{0, 2} \!+\! B_{2, 2}
);
&
  
C_{0, 2} +\!\!= M_{17};
&
C_{1, 2} +\!\!= M_{17};
&
C_{2, 2} +\!\!= M_{17};
&
C_{3, 2} +\!\!= M_{17};
\\
%%
M_{18} = ( A_{0, 0} \!+\! A_{0, 1}  )  ( B_{1, 3} \!+\! B_{3, 3}  ); &
  
C_{0, 2} -\!\!= M_{18};
&
C_{0, 3} +\!\!= M_{18};
&
C_{2, 2} -\!\!= M_{18};
&
C_{2, 3} +\!\!= M_{18};
\\
%%
M_{19}  =  ( A_{1, 0} \!+\! A_{0, 0}  )  ( B_{0, 2} \!+\! B_{2, 2} \!+\! B_{0, 3} +
B_{2, 3}  );
&
  
C_{1, 3} +\!\!= M_{19};
&
C_{3, 3} +\!\!= M_{19};
&
&
\\
%%
M_{20}  =  ( A_{0, 1} \!+\! A_{1, 1}  )  ( B_{1, 2} \!+\! B_{3, 2} \!+\! B_{1, 3} +
B_{3, 3}  );
&
  
C_{0, 2} +\!\!= M_{20};
&
C_{2, 2} +\!\!= M_{20};
&
&
\\
%%
M_{21}  =  ( A_{2, 2} \!+\! A_{3, 3}  )  ( B_{2, 0} \!+\! B_{0, 0} \!+\! B_{3, 1} +
B_{1, 1}  );
&
C_{0, 0} +\!\!= M_{21};
&
C_{1, 1} +\!\!= M_{21};
&
C_{2, 0} +\!\!= M_{21};
&
C_{3, 1} +\!\!= M_{21};
\\
%%
M_{22}  =  ( A_{3, 2} \!+\! A_{3, 3}  )  ( B_{2, 0} \!+\! B_{0, 0}  );
&
C_{1, 0} +\!\!= M_{22};
&
C_{1, 1} -\!\!= M_{22};
&
C_{3, 0} +\!\!= M_{22};
&
C_{3, 1} -\!\!= M_{22};
\\
%%
M_{23}  =  ( A_{2, 2}  )  ( B_{2, 1} \!+\! B_{0, 1} \!+\! B_{3, 1} \!+\! B_{1, 1}
);
&
C_{0, 1} +\!\!= M_{23};
&
C_{1, 1} +\!\!= M_{23};
&
C_{2, 1} +\!\!= M_{23};
&
C_{3, 1} +\!\!= M_{23};
\\
%%
M_{24}  =  ( A_{3, 3}  )  ( B_{3, 0} \!+\! B_{1, 0} \!+\! B_{2, 0} \!+\! B_{0, 0}
);
&
C_{0, 0} +\!\!= M_{24};
&
C_{1, 0} +\!\!= M_{24};
&
C_{2, 0} +\!\!= M_{24};
&
C_{3, 0} +\!\!= M_{24};
\\
M_{25} = ( A_{2, 2} \!+\! A_{2, 3}  )  ( B_{3, 1} \!+\! B_{1, 1}  ); &
C_{0, 0} -\!\!= M_{25};
&
C_{0, 1} +\!\!= M_{25};
&
C_{2, 0} -\!\!= M_{25};
&
C_{2, 1} +\!\!= M_{25};
\\
%%
M_{26}  =  ( A_{3, 2} \!+\! A_{2, 2}  )  ( B_{2, 0} \!+\! B_{0, 0} \!+\! B_{2, 1} +
B_{0, 1}  );
&
C_{1, 1} +\!\!= M_{26};
&
C_{3, 1} +\!\!= M_{26};
&
&
\\
%%
M_{27}  =  ( A_{2, 3} \!+\! A_{3, 3}  )  ( B_{3, 0} \!+\! B_{1, 0} \!+\! B_{3, 1} +
B_{1, 1}  );
&
C_{0, 0} +\!\!= M_{27};
&
C_{2, 0} +\!\!= M_{27};
&
&
\\
%%
M_{28} = ( A_{0, 0} \!+\! A_{0, 2} \!+\! A_{1, 1} \!+\! A_{1, 3}  )  ( B_{2, 2} +
B_{3, 3}  ); &
C_{0, 0} -\!\!= M_{28};
&
C_{1, 1} -\!\!= M_{28};
&
C_{0, 2} +\!\!= M_{28};
&
C_{1, 3} +\!\!= M_{28};
\\
%%
M_{29} = ( A_{1, 0} \!+\! A_{1, 2} \!+\! A_{1, 1} \!+\! A_{1, 3}  )  ( B_{2, 2}
);&
C_{1, 0} -\!\!= M_{29};
&
C_{1, 1} +\!\!= M_{29};
&
C_{1, 2} +\!\!= M_{29};
&
C_{1, 3} -\!\!= M_{29};
\\
%%
M_{30} = ( A_{0, 0} \!+\! A_{0, 2}  )  ( B_{2, 3} \!+\! B_{3, 3}  ); &
C_{0, 1} -\!\!= M_{30};
&
C_{1, 1} -\!\!= M_{30};
&
C_{0, 3} +\!\!= M_{30};
&
C_{1, 3} +\!\!= M_{30};
\\
%%
M_{31} = ( A_{1, 1} \!+\! A_{1, 3}  )  ( B_{3, 2} \!+\! B_{2, 2}  ); &
C_{0, 0} -\!\!= M_{31};
&
C_{1, 0} -\!\!= M_{31};
&
C_{0, 2} +\!\!= M_{31};
&
C_{1, 2} +\!\!= M_{31};
\\
%%
M_{32}  =  ( A_{0, 0} \!+\! A_{0, 2} \!+\! A_{0, 1} \!+\! A_{0, 3}  )  ( B_{3, 3}
);
&
C_{0, 0} +\!\!= M_{32};
&
C_{0, 1} -\!\!= M_{32};
&
C_{0, 2} -\!\!= M_{32};
&
C_{0, 3} +\!\!= M_{32};
\\
%%
M_{33} = ( A_{1, 0} \!+\! A_{1, 2} \!+\! A_{0, 0} \!+\! A_{0, 2}  )  ( B_{2, 2} +
B_{2, 3}  );&
C_{1, 1} -\!\!= M_{33};
&
C_{1, 3} +\!\!= M_{33};
&
&
\\
%%
M_{34} = ( A_{0, 1} \!+\! A_{0, 3} \!+\! A_{1, 1} \!+\! A_{1, 3}  )  ( B_{3, 2} +
B_{3, 3}  ); &
C_{0, 0} -\!\!= M_{34};
&
C_{0, 2} +\!\!= M_{34};
&
&
\\
%%
M_{35}  =  ( A_{2, 0} \!+\! A_{0, 0} \!+\! A_{3, 1} \!+\! A_{1, 1}  )  ( B_{0, 0} +
B_{0, 2} \!+\! B_{1, 1} \!+\! B_{1, 3}  );
&
C_{2, 2} +\!\!= M_{35};
&
C_{3, 3} +\!\!= M_{35};
&
&
\\
%%
M_{36}  =  ( A_{3, 0} \!+\! A_{1, 0} \!+\! A_{3, 1} \!+\! A_{1, 1}  )  ( B_{0, 0} +
B_{0, 2}  );
&
C_{3, 2} +\!\!= M_{36};
&
C_{3, 3} -\!\!= M_{36};
&
&
\\
%%
M_{37}  =  ( A_{2, 0} \!+\! A_{0, 0}  )  ( B_{0, 1} \!+\! B_{0, 3} \!+\! B_{1, 1} +
B_{1, 3}  );
&
C_{2, 3} +\!\!= M_{37};
&
C_{3, 3} +\!\!= M_{37};
&
&
\\
%%
M_{38}  =  ( A_{3, 1} \!+\! A_{1, 1}  )  ( B_{1, 0} \!+\! B_{1, 2} \!+\! B_{0, 0} +
B_{0, 2}  );
&
C_{2, 2} +\!\!= M_{38};
&
C_{3, 2} +\!\!= M_{38};
&
&
\\
%%
M_{39} = ( A_{2, 0} \!+\! A_{0, 0} \!+\! A_{2, 1} \!+\! A_{0, 1}  )  ( B_{1, 1} +
B_{1, 3}  ); &
C_{2, 2} -\!\!= M_{39};
&
C_{2, 3} +\!\!= M_{39};
&
&
\\
\multicolumn{5}{|l|}{
M_{40}  =  ( A_{3, 0} \!+\! A_{1, 0} \!+\! A_{2, 0} \!+\! A_{0, 0}  )  ( B_{0, 0} +
B_{0, 2} \!+\! B_{0, 1} \!+\! B_{0, 3}  );
} \\
&
C_{3, 3} +\!\!= M_{40};
&
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{41}  =  ( A_{2, 1} \!+\! A_{0, 1} \!+\! A_{3, 1} \!+\! A_{1, 1}  )  ( B_{1, 0} +
B_{1, 2} \!+\! B_{1, 1} \!+\! B_{1, 3}  );
}\\
&
C_{2, 2} +\!\!= M_{41};
&
&
&
\\
}
~~~~ \vdots 
&
&
&
&
\\
%%
%%
\multicolumn{5}{|l|}{
M_{42}  =  ( A_{0, 2} \!+\! A_{2, 2} \!+\! A_{1, 3} \!+\! A_{3, 3}  )  ( B_{2, 0} +
B_{2, 2} \!+\! B_{3, 1} \!+\! B_{3, 3}  );
}\\
&
C_{0, 0} +\!\!= M_{42};
&
C_{1, 1} +\!\!= M_{42};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{43}  =  ( A_{1, 2} \!+\! A_{3, 2} \!+\! A_{1, 3} \!+\! A_{3, 3}  )  ( B_{2, 0} +
B_{2, 2}  );
}\\
&
C_{1, 0} +\!\!= M_{43};
&
C_{1, 1} -\!\!= M_{43};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{44}  =  ( A_{0, 2} \!+\! A_{2, 2}  )  ( B_{2, 1} \!+\! B_{2, 3} \!+\! B_{3, 1} +
B_{3, 3}  );
}\\
&
C_{0, 1} +\!\!= M_{44};
&
C_{1, 1} +\!\!= M_{44};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{45}  =  ( A_{1, 3} \!+\! A_{3, 3}  )  ( B_{3, 0} \!+\! B_{3, 2} \!+\! B_{2, 0} +
B_{2, 2}  );
}\\
&
C_{0, 0} +\!\!= M_{45};
&
C_{1, 0} +\!\!= M_{45};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{46} = ( A_{0, 2} \!+\! A_{2, 2} \!+\! A_{0, 3} \!+\! A_{2, 3}  )  ( B_{3, 1} +
B_{3, 3}  );
}\\
 &
C_{0, 0} -\!\!= M_{46};
&
C_{0, 1} +\!\!= M_{46};
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{47}  =  ( A_{1, 2} \!+\! A_{3, 2} \!+\! A_{0, 2} \!+\! A_{2, 2}  )  ( B_{2, 0} +
B_{2, 2} \!+\! B_{2, 1} \!+\! B_{2, 3}  );
}\\
&
C_{1, 1} +\!\!= M_{47};
&
&
&
\\
%%
\multicolumn{5}{|l|}{
M_{48}  =  ( A_{0, 3} \!+\! A_{2, 3} \!+\! A_{1, 3} \!+\! A_{3, 3}  )  ( B_{3, 0} +
B_{3, 2} \!+\! B_{3, 1} \!+\! B_{3, 3}  );
}\\
&
  C_{0, 0} +\!\!= M_{48}; 
&
&
&\\ \hline
\end{array}
\]%
}
\caption{Representative computations for two levels of Strassen.}
\label{fig:2stepB}
\end{figure}

